A Linux Kernel Scheduler Extension for Multi-core Systems

The Linux kernel is mostly designed for multi-programed environments, but high-performance applications have other requirements. Such applications are run standalone, and usually rely on runtime systems to distribute the application's workload on worker threads, one per core. However, due to current OSes limitations, it is not feasible to track whether workers are actually running or blocked due to, for instance, a requested resource. For I/O intensive applications, this leads to a significant performance degradation given that the core of a blocked thread becomes idle until it is able to run again. In this paper, we present the proof-of-concept of a Linux kernel extension denoted User-Monitored Threads (UMT) which tackles this problem. Our extension allows a user-space process to be notified of when the selected threads become blocked or unblocked, making it possible for a runtime to schedule additional work on the idle core. We implemented the extension on the Linux Kernel 5.1 and adapted the Nanos6 runtime of the OmpSs-2 programming model to take advantage of it. The whole prototype was tested on two applications which, on the tested hardware and the appropriate conditions, reported speedups of almost 2x.

==> future-work.tex <==
\section{Future Work}

We plan to implement a leader-follower approach in the next iteration of
Nanos6 to minimize the number of unnecessary context switches. Also we will
study the posibility of implementing an specialized version of eventfd that
allows us to keep the count of per core ready workers on it.
Then, we will adapt an standard benchmark and a production sowftware such as
a web or database server to test the UMT mechanism.

